Credible, Optimal Auctions via Public Broadcast

We study auction design in a setting where agents can communicate over a censorship-resistant broadcast channel like the ones we can implement over a public blockchain. We seek to design credible, strategyproof auctions in a model that differs from the traditional mechanism design framework because communication is not centralized via the auctioneer. We prove this allows us to design a larger class of credible auctions where the auctioneer has no incentive to be strategic. Intuitively, a decentralized communication model weakens the auctioneer's adversarial capabilities because they can only inject messages into the communication channel but not delete, delay, or modify the messages from legitimate buyers. Our main result is a separation in the following sense: we give the first instance of an auction that is credible only if communication is decentralized. Moreover, we construct the first two-round auction that is credible, strategyproof, and optimal when bidder valuations are $\alpha$-strongly regular, for $\alpha > 0$. Our result relies on mild assumptions -- namely, the existence of a broadcast channel and cryptographic commitments.

==> 12-distributions_crypto.tex <==
We now demonstrate the necessity of considering $\alpha$-strongly regular distributions in blockchains, as opposed to simply MHR distributions.
We further provide counterexamples of items in blockchains in which the valuations of bidders are not even regular. Together, these examples allow us to situate the study of $\alpha$-strongly regular distributions that we consider in this paper.
In the subsequent, we consider that the single item for sale is a \emph{block}.
A block is a set of user transactions and the auction utilized is the proposer-builder separation defined in~\S\ref{sec:intro}.

\subsection{Constant Function Market Makers}
We now generalize sandwich attacks to more general contracts called \emph{constant function market makers}, which hold some amount of \emph{reserves} $R, R' \ge 0$ of two assets
and have a \emph{trading function} $\psi: \mathbb{R}^2\times\mathbb{R}^2 \to \mathbb{R}$.
Traders can then submit a \emph{trade} $(\Delta, \Delta')$ denoting the amount they wish to tender (if negative) or receive (if positive) from the contract.
The contract then accepts the trade if $\psi(R, R', \Delta, \Delta') = \psi(R, R', 0, 0)$,
and pays out $(\Delta, \Delta')$ to the trader.

\paragraph{Curvature.} 
We briefly summarize the main definitions and results of~\cite{angerisCurvature} here.
Suppose that the trading function $\psi$ is differentiable (as most trading functions in practice are), then
the marginal price for a trade of size $\Delta$ is
$
g(\Delta) = \frac{\partial_3 \psi(R, R', \Delta, \Delta')}{\partial_4 \psi(R, R', \Delta, \Delta')}.
$.
Here $\partial_i$ denotes the partial derivative with respect to the $i$th argument,
while $\Delta'$ is specified by the implicit condition $\psi(R, R', \Delta, \Delta') = \psi(R, R', 0, 0)$; i.e., the trade
$(\Delta, \Delta')$ is assumed to be valid. Additionally, the reserves $R, R'$ are assumed to be fixed.
Matching the notation of Section~\ref{sec:uniswap}, the function $g$ is known as the \emph{price impact} function as it represents the final marginal price of a positive-sized trade.
When there are fees, one can show that $g^{fee}(\Delta) = \gamma g(\gamma \Delta)$ where $1-\gamma$ denotes the percentage fee.
We say that a CFMM is \emph{$\alpha$-stable} if it satisfies $g(0) - g(-\Delta) \leq \alpha \Delta$
for all $\Delta \in [0, M]$ for some positive $M$.
This is a linear upper bound on the maximum price impact that a bounded trade (bounded by $M$) can have. 
Similarly, we say that a CFMM is $\beta$-liquid if it satisfies
$g(0) - g(-\Delta) \geq \beta \Delta$ for all $\Delta \in [0, K]$ for some positive $K$.
One important property of $g$ is that it can be used to compute $\Delta'$~\cite[\S2.1]{angerisCurvature}:
\begin{equation}\label{eq:curvOut}
    \Delta' = \int_{0}^{-\Delta} g(t) dt
\end{equation}
Simple methods for computing $\alpha$ and $\beta$ in common CFMMs are presented
in~\cite[\S1.1]{angerisCurvature} and~\cite[\S4]{angeris2021cfmm}. We define $G(\Delta)$ to be the \emph{forward exchange function}, which is equivalently the amount of output token received for an input of size $\Delta$. Whenever we reference the function $G(\Delta)$ for a given CFMM we always make clear the reserves associated with that function. Further, $G(\Delta)$ was shown to be concave and increasing in \cite{angeris2021cfmm}.

\paragraph{Slippage Limits.}
Analogously to the case of Uniswap, when a user submits an order to a CFMM, they submit two parameters: a trade size $\Delta \in \mathbb{R}$ and a \emph{slippage limit} $\eta \in (0, 1)$.
The slippage is interpreted as the minimum output amount that the user is willing to accept as a fraction of $G(\Delta)$. That is, the trade is accepted if the amount in output token the user receives is larger than or equal to $(1-\eta) G(\Delta)$.
However, the majority of this paper will focus on representing slippage limits in quantity space (e.g. in terms of $G(\Delta)$ not $g(\Delta)$).

\paragraph{Valuations in CFMMs}
In Flashbots' MEV auction, decentralized exchange arbitrage transactions are amongst the most bid upon transactions with over \$1 billion of MEV profits generated~\cite{flashbots_mev_explore}.
One particular type of transaction, the sandwich attack, has been formally studied and generic bounds of profitability have been constructed~\cite{kulkarni2022towards}.
We can use these bounds on profitability to construct a valuation for sandwich attacks.
\cite{kulkarni2022towards}~shows the following bound for the profit of sandwiching a single trade $\Delta$ with slippage limit $\eta$:
\[
    \mathsf{PNL}(\Delta, \eta) \leq  \left(O(\eta) + \gamma - 1\right)\Delta - \frac{\mu\gamma}{\beta} \leq C \max(\eta, \sqrt{1+\eta}) \Delta - \frac{\mu\gamma}{\beta}
\]
As such, if we receive a sequence of trades $(\Delta_1, \eta_1), \ldots, (\Delta_n, \eta_n)$, we can write a user's valuation $\nu_i$ for the sequence of trades as
\[
\nu_i((\Delta_1, \eta_1), \ldots, (\Delta_n, \eta_n)) = \sum_{i=1}^n \mathsf{PNL}(\Delta_i, \eta_i)
\]
Assuming that the trades $(\Delta_i, \eta_i)$ are drawn jointly from a distribution $P$, given a total trade volume $V$, we define the valuation for an MEV searcher (who is an auction bidder) for a given volume as
\[
v_i(V) = \Expect_{
(\Delta_i, \eta_i) \sim P}\left[ \nu_i((\Delta_1, \eta_1), \ldots, (\Delta_n, \eta_n)) \vert \sum_i \Delta_i = V \right]
\]
\paragraph{Values for CFMMs are generically strongly regular}
We now demonstrate that for a sequence of CFMM trades, with total trade volume $V$, $v(V)$ is generically strongly regular given that the trades are sampled iid from a strongly regular distribution. Further, we assume that there exist constants $\mu, \gamma, \beta$ corresponding to a CFMM. We make the following assumption on the trade-generating distribution $P$: the trades $\Delta \in \mathbf{R}^n$ drawn jointly from $P$ can be written as: 
\begin{align*}
    \Delta = D_1 \mathbf{e_1} + \dots + D_n \mathbf{e_n} \\
\end{align*}
where $D_i$ are sampled iid from a strongly regular distribution, $\mathbf{e_i}$ are the basis vectors in $\mathbf{R}^n$, and the slippage limits $\eta_i$ are chosen deterministically. By noting that the value $\nu_i((\Delta_1, \eta_1), \dots, (\Delta_n, \eta_n)) = \sum_{i=1}^{n} \mathsf{PNL}(\Delta_i, \eta_i)$, we therefore have that: 
\begin{align*}
    \sum_{i=1}^{n} \mathsf{PNL}(\Delta_i,\eta_i) \leq C \max(\eta_i, \sqrt{1+\eta_i} \sum_{i=1}^{n} \Delta_i - \frac{n \mu \gamma}{\beta}
\end{align*}
Noting that $\sum_{i=1}^n \Delta_i$ is also strongly regular, and that scaled and shifted strongly regular distributions are also strongly regular, we have that $v_i(V)$ is strongly regular. 
\paragraph{Example of non-MHR Distribution in CFMMs} We now construct an explicit example of a value distribution in CFMMs that is regular but not MHR. Intuitively, this occurs when the distribution of trades is 'heavy tailed', which occurs in decentralized exchanges on blockchains, especially in times of high market volatility. We assume that blocks of size $1$, in which a user's trade $\Delta_1$ is drawn from a distribution $F$ with density $f(x) = \frac{1}{(1+x)^2}$ and the slippage $\eta_1$ is deterministic and known. Then, we have that the valuation for the MEV searcher is given by:
\begin{align*}
    v(V) &= \Expect_{\Delta_1 \sim F} \left[ \mathsf{PNL}(\Delta_1, \eta_1) | \Delta_1 = V \right] \\ & \leq C \max (\eta, \sqrt{1+\eta}) 
    \Expect_{\Delta_1 \sim F} [\Delta_1] - \frac{\mu \gamma}{\beta}
\end{align*}
Defining the constants $a = C \max (\eta, \sqrt{1+\eta})$ and $b =  \frac{\mu \gamma}{\beta}$, we therefore want to show that $\mathsf{PNL}(\Delta_1, \eta_1)$ is not distributed according to an MHR distribution. To do this, we first show that $a \Delta_1 - b$ is not MHR. This follows from standard results on scaling and shifting non-MHR distributions. The key step is showing that $f(x) = \frac{1}{(1+x)^2}$ is not MHR. Computing the virtual value, $\varphi(x)$, and noting that $F$ has CDF $F(x) = 1-\frac{1}{1+x}$, we have: 
\begin{align*}
    \varphi(x) & = x - \frac{1-F(x)}{f(x)} \\ & = x - \frac{1 - \left( 1 - \frac{1}{1+x} \right)}{(1+x)^2} \\ & = x - (1+x) \\ & = -1
\end{align*}
This clearly does not satisfy the condition for being MHR. 

\subsection{Liquidations} 
% We now show how the above (benign) characterization of the value distribution for a transaction set that only contains transactions from CFMMs may differ drastically from a transaction set corresponding to on-chain liquidations, and hence, any auction designed for such a transactions must account for value distributions that are not well-behaved. 
A liquidation is a transaction that is specified by two assets, called the \emph{collateral} (C) and \emph{debt} (D). We denote the current price of the two assets as $p_C$ and $p_D$, where we normalize $p_C= 1$, and therefore $p_D$ is the price of the debt asset in units of collateral. A smart contract on a blockchain such as Ethereum has lent out some amount of $D$ in exchange for holding $C$ as collateral for the debt. Let $x_C$ denote the amount of collateral and $x_D$ the amount of debt. As a result of price change of the debt asset relative to the collateral, the debt may become \emph{liquidatable}. In particular, if the debt-to-collateral ratio $\frac{x_D p_D}{x_C}$ is less than 1, the debt is called healthy. Otherwise, the debt is called liquidatable. We denote the tuple $L= (p_D, x_C, x_D)$ as a liquidation. The prices $p_C$ and $p_D$ are random variables that we describe in more detail subsequently. We write $\mathbbm{1}_L \in \{0,1\}$ to denote the liquidatability of the debt. If $\mathbbm{1}_L = 0$, then the debt is healthy, and else it is liquidatable.

\paragraph{Liquidations are not regular} 
We now demonstrate that the valuations for liquidations are not regular. Recall that liquidations have value functions $v(L) = \mathbbm{1}_{L}$ where $\mathbbm{1}_L =1$ if $x_D p_D/x_C > 1$ and $0$ otherwise. Assume without loss of generality that $x_D = x_C = 1$, and that $p_D \sim \mathcal{N}(1,1)$. We therefore see that $\mathbbm{1}_L = 1$ with probability $0.5$ and $\mathbbm{1}_L = 0$ with probability $0.5$. This value distribution is not even regular, because $f(x) = 0.5 \delta(x) + 0.5\delta(x-1)$, which gives us:
\begin{align*}
    F(x) = \begin{cases}
        0.5 \text{ if } 1 > x \geq 0 \\
        1 \text{ if } x \geq 1 
    \end{cases}
\end{align*}
Consider $x, x' = 0, 0.5$. Then, we have $\phi(0) = \frac{1-0.5}{0.5}$ and $\phi(0.5) = 0.5 - \frac{1 - 0.5}{0} = -\infty$. Therefore, we clearly do not have $\phi(0.5) - \phi(0) \geq 0$.
%\end{document}


==> 13-lemma-6.tex <==
We include here the proof of Lemma \ref{lemma:small-collateral}. 

\begin{proof}
When $v_j < \beta_j(\vec v)$ for all buyers, a false buyer is the highest bidder. Therefore, $\max_j \beta_j(\vec v) = \tilde b(n, D) > f(n, D)$ where the inequality is a statement assumption. In this case, any real buyer can receive the item as long as the auctioneer withholds at least one bid. Because buyer $j$ pays at most $v_j$, the auctioneer receives negative revenue if $v_j < f(n, D)$. Recall $x_i(\vec v)$ is an indicator variable taking value $1$ if and only if buyer $i$ receives the item. This gives
%
\begin{align*}
& \e[\vec v \leftarrow D]{R(\vec v) \cdot \ind{\forall j, v_j < \beta_j(\vec v)}}\\
&\qquad\leq \e[v \leftarrow D]{\sum_{i = 1}^n (v_i - f(n, D)) \cdot x_i(\vec v) \cdot \ind{\forall j, v_j < \beta_j(\vec v)} \cdot \ind{v_i \geq f(n, D)}}\\
&\qquad\leq \e[\vec v \leftarrow D]{\sum_{i = 1}^n \left(\frac{1}{\alpha}\varphi(v_i) + r(D) - f(n, D)\right) \cdot x_i(\vec v) \cdot \ind{\forall j, v_j < \beta_j(\vec v)} \cdot \ind{v_i \geq f(n, D)}}\\
&\qquad\leq \e[\vec v \leftarrow D]{\sum_{i = 1}^n \frac{1}{\alpha}\varphi(v_i) \cdot x_i(\vec v) \cdot \ind{\forall j , v_j < \beta_j(\vec v)} \cdot \ind{v_i \geq f(n, D)}}\\
&\qquad= \e[\vec v \leftarrow D]{\sum_{i = 1}^n \frac{1}{\alpha}\varphi(v_i) \cdot x_i(\vec v) \cdot \ind{\forall j \neq i, v_j < \beta_j(\vec v)} \cdot \ind{f(n, D) \leq v_i < \beta_i(\vec v)}}\\
&\qquad= \e[\vec v \leftarrow D]{\sum_{i = 1}^n \frac{\varphi(v_i)}{\alpha} \cdot x_i(\vec v) \cdot \ind{\forall j \neq i, v_j < \beta_j(\vec v)} \cdot (\ind{v_i \geq f(n, D)} - \ind{v_i > \beta_i(\vec v)})}\\
&\qquad < \e[\vec v \leftarrow D]{\sum_{i = 1}^n \frac{\varphi(v_i)}{\alpha} \cdot \ind{v_i \geq f(n, D)}} - \e[\vec v \leftarrow D]{\sum_{i = 1}^n \varphi(v_i) \cdot \ind{v_i > \beta_i(\vec v)}}
\end{align*}
%
The second line observes that if buyer $i$ receives the item, they pay at most $v_i$, and the auctioneer loses a collateral of $f(n, D)$ by withholding at least one bid. The third line invokes Lemma~\ref{lemma:alpha-regular}. To see that the assumptions for the Lemma are satisfied, let $E$ be the event where $v_i \geq f(n, D)$ and observe that $f(n, D) \geq r(D)$ for all $n \geq 1$ and $\alpha \in (0, 1)$. The fourth line observes $f(n, D) \geq r(D)$. The fifth line observes the event $\{\forall j, v_j < \beta_j(\vec v)\}$ implies $\{v_i < \beta_i(\vec v)\}$ and uses the fact $\beta_i(\vec v) > f(n, D)$. The sixth line uses the fact $\ind{a \leq X < b} = \ind{X \geq a} - \ind{X \geq b}$ for any random variable $X$ and constants $a > b$. The seventh line uses the fact $\alpha > 1$ and Observation~\ref{obs:single-candidate} which states the event $\{v_i > \beta_i\}$ implies $x_i(\vec v)$ and $v_j < \beta_j(\vec v)$ for all $j \neq i$ since $v_i$ expects to win the item. Moreover, we use the fact 
%
$$x_i(\vec v) \cdot \ind{\forall j \neq i, v_j < \beta_j(\vec v)} \cdot \ind{v_i \geq f(n, D)} \leq \ind{v_i \geq f(n, D)}.$$

To conclude, we must show that
\begin{align*}
    \e[\vec v \leftarrow D]{\sum_{i = 1}^n \frac{\varphi(v_i)}{\alpha} \cdot \ind{v_i \geq f(n, D)}} \leq \rev(D^n).
\end{align*}
%
From Lemma~\ref{lemma:single-revenue-upper-bound},
\begin{align*}
&\e[\vec v \leftarrow D]{\sum_{i = 1}^n \frac{\varphi(v_i)}{\alpha} \cdot \ind{v_i \geq f(n, D)}}\\
&\qquad= \frac{1}{\alpha}\left(\frac{1}{1-\alpha}\right)^{\frac{1}{1-\alpha}} \left(\frac{r(D)}{f(n, D)}\right)^{\frac{\alpha}{1-\alpha}}\e[\vec v \leftarrow D]{\sum_{i = 1}^n \varphi(v_i) \cdot \ind{v_i \geq r(D)}}\\ 
&\qquad\leq \frac{\alpha}{\alpha n}\e[\vec v \leftarrow D]{\sum_{i = 1}^n \varphi(v_i) \cdot \ind{v_i \geq r(D)}} \\
&\qquad = \frac{\alpha n}{\alpha n} \e[v_1 \leftarrow D]{\varphi(v_1) \cdot \ind{v_1 \geq r(D)}}\\
&\qquad = \rev(D)\\
&\qquad \leq \rev(D^n)
\end{align*}
%
The second line observes $f(n, D) \geq r(D)$ and applies Lemma~\ref{lemma:single-revenue-upper-bound}. The third line uses the assumption $f(n, D) \geq r(D) \left(\frac{n}{\alpha}\right)^{\frac{1-\alpha}{\alpha}}\left(\frac{1}{1-\alpha}\right)^{\frac{1}{\alpha}}$. The fourth line observes $\varphi(v_1), \ldots, \varphi(v_n)$ are i.i.d.. The fifth line observes $r(D)$ is the optimal reserve price, and so $\e[v_1 \leftarrow D]{\varphi(v_1) \cdot \ind{v_1 \geq r(D)}}$ is the optimal revenue for the single buyer auction (Theorem~\ref{thm:myerson}). The last line observes the revenue is non-decreasing in the number of buyers.
\end{proof}

==> 7-applications.tex <==


%%% Use for ArXiv Version only
% \documentclass[12pt, class=article, crop=false]{standalone}

% \usepackage{preample}

% \begin{document}

In this section, we introduce various applications of credible auctions. We discuss auctions for non-fungible tokens (NFTs), and auctions for the block construction process (to auction off application-layer value called MEV) and proposer-builder separation .

\paragraph{NFTs.}
Non-fungible tokens (NFTs) are data structures that can be used to represent a unique, non-divisible asset.
Commonly, NFTs are used to represent art and/or collectibles, and users purchase NFTs with fungible tokens such as Ethereum and/or stablecoins---tokenized representations of currencies such as dollars.
Most NFTs are transferred via auctions on platforms like OpenSea, with tens of billions of dollars of auction volume since 2020.
NFT auctions have been studied formally and demonstrated that they could not satisfy strategyproofness and collusion resistance if auctioneer-buyer coalitions share full information~\cite{milionis2022framework}.
One natural question is if one can design a credible auction.
Indeed, $\dra$ can provide strong security guarantees for users for a broader class of distributions.

\paragraph{Maximal Extractable Value.}
Validators are responsible for choosing which transactions will enter the blockchain.
Because blockchain space is a scarce resource, validators set up an auction for blockspace.
These auctions have become increasingly competitive because agents can obtain monetary profits by reordering, adding, or removing transactions that enter the blockchain.
The largest possible profits often called maximal extractable value (MEV).
Since 2020, most MEV has been extracted via coordinated auctions run by validators, with the most popular auction being the Flashbots auction~\cite{flashbots_mev_explore}.
Flashbots, in particular, have generated billions of dollars of auction revenue for validators.
Bidders in these auctions, known as MEV searchers, bid on transaction priority for sequences of transactions.
For instance, a bidder who sees a publicly posted Ethereum transaction for a trade may enter the auction with a bundle consisting of a front-run transaction plus the public user transaction.
If a bidder wins an auction, they are guaranteed that their bundle of transactions is included in the block, and the auction revenue is distributed to the validator who proposed that successful block.
These auctions and MEV have been studied in several works that analyzed empirical auction performance~\cite{daian2020flash, weintraub2022flash}, theoretical properties such as the price of anarchy~\cite{kulkarni2022towards}, optimal bidding strategies~\cite{angeris2021note}, and mechanisms for reducing auction revenue~\cite{ferreira2022credible, mcmenamin2022fairtradex, kelkar2022order, cachin2022quick}. Recent work has also considered the problem of designing transaction fee mechanisms that are incentive compatible for both users and block producers when the block producers have additional private value for user transactions \cite{bahrani2023transaction}.

Currently, these auctions are run as sealed-bid, first-price auctions\footnote{We note that there are side-channels for reading auction bids that often render these auctions not sealed-bid in practice, as adversaries with enough resources can learn your bids. However, most of the documentation on these auctions describes them as `sealed-bid' in that the auctioneer does not share the bids with other bidders, even after an auction has been completed.} run by a monopolist.
However, there has been a desire to decentralize this auction such that no single entity controls transaction inclusion~\cite{MEV_Suave}.
One motivation is that a centralized auctioneer can censor particular transactions and/or delay the confirmation of time-sensitive transactions.
The act of decentralizing such auctions such that no single auctioneer can manipulate the outcome is tantamount to having a credible, truthful, censorship-resistant auction. 
Moreover, to ensure the liveness of the underlying blockchain---its ability to continue to accept transactions---, one needs bounded communication complexity.

Flashbots explicitly asks for this in their early design of their decentralized auction~\cite{kilbourn_2022}:
\begin{quote}
If inclusion is not monopolized [...] it might be the case that the sequence of auctions is important in determining where value flows [...] the designs explored in this article feature two auctions, with the first executed without ``full information''. Is it possible to design a single incentive-compatible, credible auction that takes into account more information?
\end{quote}

The DRA presented in~\S\ref{sec:dra} is, to the authors' best knowledge, the first auction to meet these requirements in the blockchain setting with independent private valuations. The consideration of $\alpha$-strongly regular distributions for $\alpha \in (0,1)$ is relevant in these auctions, as in the case of a class of decentralized exchanges called constant function market makers (CFMMs)~\cite{angeris2021cfmm}.  Further, most MEV auctions that run on blockchains occur in transactions originating from CFMMs~\cite{flashbots_mev_explore}. Transaction types called liquidations (which occur on most blockchains) whose values are not even regular, and demonstrate that DRA is not credible for these transactions which comprise non-trivial revenue within MEV auctions. Thus, considering $\alpha$-strongly regular distributions for various values of $\alpha$ is relevant in maximal extractable value auctions. 

\paragraph{Proposer-Builder Separation.}
While an MEV auction is often defined as a combinatorial auction where bidders have valuations for distinct transaction bundles, there exist other blockchain auctions that involve selling a single item.
MEV auctions are primarily run outside of the consensus mechanism of a blockchain that determines the validity of a new sequence of transactions.
This is because it is not possible for a decentralized network to come to an agreement on particular orderings (i.e.,~this problem reduces to ranked voting, and Arrow's impossibility theorem applies~\cite{kelkar2022order}).

On the other hand, new consensus mechanisms enable a validator to delegate block building to another party allowing the validator to auction an entire block. For example, Proof-of-Work requires the block to be determined before validator selection.
On the other hand, Proof-of-Stake allows the block content to be determined after the validator is selected~\cite{ferreira2021proof, ferreira2022optimal}.
Thus the validator selected can auction away the privilege to build the next block  by receiving offers $(b, B)$ where $b \in \mathbb{R}_+$ is a bid and $B$ is a valid block.
These are single-item auctions, where the auctioneer is selling the right for $B$ to become the next block. 
This separation between the proposer (the winner of the lottery to become the next block proposer) and the builder (the bidder submitting valid blocks) is meant to increase the decentralization of block production in blockchains~\cite{bahrani2023transaction}.

Until now, it has not been formally known if such a scheme can be made incentive compatible.
Prior heuristic analysis by~\cite{buterin_2021} demonstrates that the cost of censorship (e.g., forcing a particular bid to not win in spite of being the highest bid) decreases in the PBS model.
However, this model did not account for the auctioneer (the proposer) also participating in the auction and adding fake bids.
The collateral requirements for the DRA of \S\ref{sec:dra} can be used to formally realize the censorship-resistant bounds of~\cite{buterin_2021}.
Moreover, the credibility of this auction ensures that even if the auctioneer deviates, provided that the PBS auction follows a DRA and user valuations are $\alpha$-strongly regular, private, and independent, then PBS is robust to censorship.
%\end{document}
